Autoencoder Based Deep Clustering of Point Clouds

Motivated by a problem in Generative Specification-Producing AIs (SPAIs), we focus on a problem of deep clustering of three-dimensional shapes specified by point clouds. After reviewing clustering and deep clustering, we study the fully unsupervised pipeline in which a FoldingNet autoencoder is first trained for reconstruction and then K-means++ is then applied to the resulting codewords. We report clustering accuracy (ACC), normalized mutual information (NMI) and adjusted Rand index (ARI) on ModelNet10 and ModelNet40 datasets, as a function of the number of clusters K. We also provide t-SNE visualizations of the codewords, and discuss the choice of K.

==> tables/kmeans_distortion_modelnet10.tex <==
2 & 139.7761 & -3247765.9 \\
4 & 113.4466 & -3762568.4 \\
6 & 99.6099 & -4080123.6 \\
8 & \textbf{90.3852} & -4315180.3 \\
10 & 85.2159 & -4454198.2 \\
12 & 81.1808 & -4567172.7 \\
14 & 77.5610 & -4672887.0 \\
16 & 74.7198 & -4757794.4 \\
18 & 72.1471 & -4836979.8 \\
20 & 70.1984 & \textbf{-4896959.1} \\


==> tables/kmeans_distortion_modelnet40.tex <==
10 & 38.9346 & -16191691.4 \\
20 & 31.6331 & -17452510.0 \\
30 & 27.8940 & -18197201.8 \\
35 & \textbf{26.5951} & -18473647.2 \\
40 & 25.6435 & -18679197.8 \\
45 & 24.7859 & -18869500.5 \\
50 & 23.9902 & -19051052.2 \\
60 & 22.6855 & -19355311.0 \\
70 & 21.7054 & -19585483.1 \\
80 & 20.8521 & \textbf{-19790065.6} \\

